Audio-Synchronized Visual Animation

Current visual generation methods can produce high quality videos guided by texts. However, effectively controlling object dynamics remains a challenge. This work explores audio as a cue to generate temporally synchronized image animations. We introduce Audio Synchronized Visual Animation (ASVA), a task animating a static image to demonstrate motion dynamics, temporally guided by audio clips across multiple classes. To this end, we present AVSync15, a dataset curated from VGGSound with videos featuring synchronized audio visual events across 15 categories. We also present a diffusion model, AVSyncD, capable of generating dynamic animations guided by audios. Extensive evaluations validate AVSync15 as a reliable benchmark for synchronized generation and demonstrate our models superior performance. We further explore AVSyncDs potential in a variety of audio synchronized generation tasks, from generating full videos without a base image to controlling object motions with various sounds. We hope our established benchmark can open new avenues for controllable visual generation. More videos on project webpage https://lzhangbj.github.io/projects/asva/asva.html.

==> equations/a2v_diffusion_step.tex <==
% \abovedisplayskip=3pt
% \abovedisplayshortskip=3pt
% \belowdisplayskip=3pt
% \belowdisplayshortskip=3pt
\begin{equation}
    [ \boldsymbol{z}_1^{t-1}, \boldsymbol{z}_2^{t-1}, ..., \boldsymbol{z}_f^{t-1} ] = 
    \text{Diffuse}(
        [ \boldsymbol{z}_1, \boldsymbol{z}_2^{t}, ..., \boldsymbol{z}_f^{t} ],
        t,
        \boldsymbol{\theta}
        )
\end{equation}

==> equations/audio_xattn.tex <==
\begin{align}
    \boldsymbol{q}_k = \text{Linear}(\boldsymbol{z}_k), \boldsymbol{k}_k &= \text{Linear}(\boldsymbol{c}_k), \boldsymbol{v}_k = \text{Linear}(\boldsymbol{c}_k) \\
    \boldsymbol{z}_k &= \text{Attention}(\boldsymbol{q}_k, \boldsymbol{k}_k, \boldsymbol{v}_k)
\end{align}

==> equations/first_frame_condition_conv.tex <==
\begin{equation}
    \boldsymbol{e}_k = \text{Linear}(\boldsymbol{e}_0, \boldsymbol{e}_{k-1}, \boldsymbol{e}_k)
\end{equation}

==> equations/text_to_image_equation.tex <==
\begin{equation}
    \textit{L} := \mathbb{E}_{\mathcal{E}(\boldsymbol{x}), \epsilon\sim \textit{N}(0, 1), t}(\| \epsilon - \epsilon_{\theta}(\boldsymbol{z}^t, t, \boldsymbol{\tau})  \|)
\end{equation}

==> figures/all_category_qualitative_view.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.7\linewidth]{figures/images/all_category_qualitative_view.png}
    \caption{Generated samples by A2VD on each category.}
    \label{fig:all_category_qualitative_view}
\end{figure*}
